MonoPatchNeRF: Improving Neural Radiance Fields with Patch-based Monocular Guidance

The latest regularized Neural Radiance Field (NeRF) approaches produce poor geometry and view extrapolation for large scale sparse view scenes, such as ETH3D. Density-based approaches tend to be under-constrained, while surface-based approaches tend to miss details. In this paper, we take a density-based approach, sampling patches instead of individual rays to better incorporate monocular depth and normal estimates and patch-based photometric consistency constraints between training views and sampled virtual views. Loosely constraining densities based on estimated depth aligned to sparse points further improves geometric accuracy. While maintaining similar view synthesis quality, our approach significantly improves geometric accuracy on the ETH3D benchmark, e.g. increasing the F1@2cm score by 4x-8x compared to other regularized density-based approaches, with much lower training and inference time than other approaches.

==> figures/eth3d_acmmp.tex <==
\begin{figure}
\centering
\includegraphics[width=0.31\textwidth]{images/eth3d_rendering/courtyard.png}
\includegraphics[width=0.31\textwidth]{images/eth3d_rendering/delivery_area.png}
\includegraphics[width=0.31\textwidth]{images/eth3d_rendering/electro.png}
\includegraphics[width=0.31\textwidth]{images/eth3d_rendering/facade.png}
\includegraphics[width=0.31\textwidth]{images/eth3d_rendering/kicker.png}
\includegraphics[width=0.31\textwidth]{images/eth3d_rendering/meadow.png}
\includegraphics[width=0.31\textwidth]{images/eth3d_rendering/pipes.png}
\includegraphics[width=0.31\textwidth]{images/eth3d_rendering/office.png}
\includegraphics[width=0.31\textwidth]{images/eth3d_rendering/playground.png}
\includegraphics[width=0.23\textwidth]{images/eth3d_rendering/relief.png}
\includegraphics[width=0.23\textwidth]{images/eth3d_rendering/relief_2.png}
\includegraphics[width=0.23\textwidth]{images/eth3d_rendering/terrace.png}
\includegraphics[width=0.23\textwidth]{images/eth3d_rendering/terrains.png}
\caption{\textbf{Training View renderings of ETH3D with MVS Depth guidance.} 
    We render mesh, color and normals of the training views of model trained with MVS guidance.
    We show that the rendered geometry and appearance are accurate and detailed.
}
\label{fig:eth3d_acmmp}
\end{figure}

==> figures/eth3d_depth_maps.tex <==
\begin{figure}
\centering
\begin{tabular}{c@{\hspace{1.0mm}}c@{\hspace{1.0mm}}c@{\hspace{1.0mm}}c}
        \includegraphics[width=0.24\textwidth]{images/depths/courtyard_rgb.png} &
        \includegraphics[width=0.24\textwidth]{images/depths/courtyard_gt.png} &
        \includegraphics[width=0.24\textwidth]{images/depths/courtyard_omnidata.png} &
        \includegraphics[width=0.24\textwidth]{images/depths/courtyard_none.png} \\
        RGB & G.T. & Prior & None \\
        \includegraphics[width=0.24\textwidth]{images/depths/courtyard_cull.png} &
        \includegraphics[width=0.24\textwidth]{images/depths/courtyard_mono.png} &
        \includegraphics[width=0.24\textwidth]{images/depths/courtyard_both.png} &
        \includegraphics[width=0.24\textwidth]{images/depths/courtyard_all.png}\\
        Restr. & Mono. & Novel & All
        
\end{tabular}
\caption{
\textbf{Visualization of depth maps for different ablations.} 
We visualize the test view of the ETH3D \textit{Courtyard} scene for comparison. 
From the top left, RGB image, ground truth depth~(G.T.), monocular prior~(Prior), base configuration~(None), with density restriction~(Restr.), with monocular geometry distillation~(Mono), with novel view patch regularization~(Novel) and with all contributions~(All). 
}
\label{fig:eth3d_depths}
\end{figure}

==> figures/overview.tex <==
\begin{figure}
    \centering
    \includegraphics{}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

==> figures/tnt.tex <==
% \begin{figure*}
% % \includegraphics[width=.99\textwidth]{images/architectures/network_structure.pdf}
% \centering
% \begin{tabular}{c@{\hspace{3mm}}c@{\hspace{3mm}}c}
%         % \includegraphics[width=0.235\textwidth]{images/teaser_fiture_rgb_comparison/combination/median/freenerf_median.png} &       
%         % \includegraphics[width=0.20\textwidth]{images/teaser_fiture_rgb_comparison/freenerf_courtyard_000030.rgb.png}&
%         {\includegraphics[trim=0cm 4.8cm 0cm 4.2cm, clip, width=0.30\textwidth, height=0.228\textwidth]{images/tnt/church_2.png}}&
%         {\includegraphics[trim=1.0cm 2.0cm 0cm 7.0cm, clip, width=0.30\textwidth, height=0.228\textwidth]{images/tnt/barn.png}} &
%         \includegraphics[width=0.30\textwidth, height=0.228\textwidth]{images/tnt/meetingroom.png} \\
%         % \includegraphics[width=0.45\textwidth, height=0.228\textwidth]{images/tnt/courthouse.png}\\
%         \multicolumn{2}{c}{Rendered image} & Point cloud
        
% \end{tabular}
% \vspace{-0.05in}
%     \caption{\textbf{Free-form views rendering and point clouds visualization for TnT~\cite{knapitsch2017tanks}.} 
%     The first and second row show rendered image and point cloud of indoor and outdoors scenes respectively. 
%     Our method generates high-quality rendered images with detailed texture and accurate geometry in densely captured large-scale scenes. 
% }
% \label{fig:tnt_qualitative}
% \vspace{-0.15in}
% \end{figure*}
\begin{figure*}
% \includegraphics[width=.99\textwidth]{images/architectures/network_structure.pdf}
\centering
\begin{tabular}{c@{\hspace{3mm}}c}
        % \includegraphics[width=0.235\textwidth]{images/teaser_fiture_rgb_comparison/combination/median/freenerf_median.png} &       
        % \includegraphics[width=0.20\textwidth]{images/teaser_fiture_rgb_comparison/freenerf_courtyard_000030.rgb.png}&
        {\includegraphics[trim=0cm 4.8cm 0cm 4.2cm, clip, width=0.45\textwidth, height=0.228\textwidth]{images/tnt/church_2.png}}&
        % \includegraphics[width=0.30\textwidth, height=0.228\textwidth]{images/tnt/meetingroom.png} \\
        \includegraphics[width=0.45\textwidth, height=0.228\textwidth]{images/tnt/meetingroom.png} \\
        {\includegraphics[trim=1.0cm 2.0cm 0cm 7.0cm, clip, width=0.45\textwidth, height=0.228\textwidth]{images/tnt/barn.png}} &
        \includegraphics[width=0.45\textwidth, height=0.228\textwidth]{images/tnt/courthouse.png}\\
        Rendered image & Point cloud
        
\end{tabular}
\vspace{-0.05in}
    \caption{\textbf{Free-form views rendering and point clouds visualization for TnT~\cite{knapitsch2017tanks}.} 
    The first and second row show rendered image and point cloud of indoor and outdoors scenes respectively. 
    Our method generates high-quality rendered images with detailed texture and accurate geometry in densely captured large-scale scenes. 
}
\label{fig:tnt_qualitative}
\vspace{-0.15in}
\end{figure*}

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> tables/monosdf.tex <==
\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|cccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{PSNR $\uparrow$} & \multirow{2}{*}{SSIM $\uparrow$} & \multirow{2}{*}{LPIPS$\downarrow$} & Prec.$_{2cm}$ $\uparrow$ & Recall$_{2cm}$ $\uparrow$ & F-score$_{2cm}$ $\uparrow$ & F-score$_{5cm}$ $\uparrow$ \\
&&&& \small{Mean / In / Out} &  \small{Mean / In / Out} & \small{Mean / In / Out} & \small{Mean / In / Out}\\
\midrule
MonoSDF_{1.0} & 15.56 & 0.598 & 0.609 & 10.8 / 19.2 / 1.1 & 17.4 / 23.4 / 10.5 & 12.0 / 20.6 / 1.8 & 21.7 / 31.9 / 9.9 \\
MonoSDF_{0.1} & 18.85 & 0.679 & 0.498 & \f{25.2} / 26.2 / \f{24.0} & 19.3 / 28.5 / 8.5 & 20.1 / 26.9 / 12.1 & 41.1 / 45.2 / 36.4 \\
\midrule
Ours & \f{20.12} & \f{0.720} & \f{0.379} & 24.4 / \f{29.8} / 18.2 &  \f{36.2} / \f{45.6} / \f{25.2} & \f{28.8} / \f{35.6} / \f{20.9} & \f{46.9} / \f{52.9} / \f{40.0} \\
\midrule
\end{tabular}
}
\caption{
    \textbf{Comparison of MonoSDF~\cite{yu2022monosdf} performance with different bias values.}
    MonoSDF$_{1.0}$ denotes MonoSDF trained with the default bias parameter~(1.0) in the code provided by the authors on the large scale TnT~\cite{knapitsch2017tanks} evaluation. MonoSDF$_{0.1}$ denotes MonoSDF trained with the parameter suggested by the authors~(0.1) for large-scale scenes specifically. 
}
\label{tab:monosdf}
\end{table*}



==> tables/monosdf_eth3d.tex <==
\begin{table*}[h]
\caption{
    \textbf{Comparison of MonoSDF~\cite{yu2022monosdf} performance with different bias values.}
    We report F-score$_{2cm}$ for all ETH3D~\cite{schops2017multi} scenes for the baselines, MonoSDF with varying bias parameters and our method. 
    MonoSDF$_{1.0}$ denotes MonoSDF trained with the default bias parameter~(1.0) in the code provided by the authors on the large scale TnT~\cite{knapitsch2017tanks} evaluation. MonoSDF$_{0.1}$ denotes MonoSDF trained with the parameter suggested by the authors~(0.1) for large-scale scenes specifically. 
}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccccccccccc|c}
\toprule
Method & Courtyard & Delivery Area & Electro & Facade & Kicker & Meadow & Office & Pipes & Playground & Relief & Relief 2 & Terrace & Terrains & Mean \\
\midrule
RegNeRF & 2.7 & 1.6 & 1.8 & 1.6 & 28.9 & 2.1 & 1.3 & 1.0 & 3.6 & 12.7 & 11.1 & 1.4 & 13.6 & 6.4\\
FreeNeRF & 6.9 & 0.7 & 0.0 & 3.1 & 19.6 & 0.1 & 4.6 & 4.5 & 0.0 & 0.9 & 1.7 & 0.2 & 0.6 & 3.3 \\
MonoSDF_{1.0} & 9.4 & 0.0 & 0.0 & 1.6 & 38.3 & 0.0 & 58.3 & 47.8 & 0.0 & 0.1 & 0.0 & 0.0 & 0.0 & 12.0 \\
MonoSDF_{0.1} & 16.1 & 14.6 & 11.7 & 3.4 & 36.2 & 10.2 & 6.9 & 27.5 & 0.0 & 37.5 & 38.6 & 31.3 & 27.2 & 20.1\\
\midrule
Ours & 17.8 & 14.5 & 13.0 & 10.6 & 63.5 & 42.2 & 21.2 & 16.4 & 12.3 & 42.3 & 46.8 & 29.6 & 44.5 & 28.8 \\
\midrule
\end{tabular}
}
\label{tab:monosdf_eth3d}
\end{table*}



==> tables/timing.tex <==
% \begin{table}[h]
% \begin{small}
% \centering
% % \renewcommand{\arraystretch}{0.9}
% \begin{tabular}{@{}c|cc@{}}
%     \toprule
%     % header
%     Model & \# Steps & Time~(hh:mm)  \\
%     \midrule
%     FreeNeRF~\cite{yang2023freenerf} & 200,000 & 14:26 & 36.4\\
%     RegNeRF~\cite{niemeyer2022regnerf} & 200,000 & 07:00 & 30.4\\
%     MonoSDF~\cite{yu2022monosdf} & 200,000 & 20:54 & 137\\
%     Neuralangelo~\cite{li2023neuralangelo} & 200,000 & 19:58 & 61.9\\
%     Ours & 50,000 & 02:15 & 3.0\\
%     \bottomrule
    
% \end{tabular}
% \caption{
%     \textbf{Training and Inference Time.} We report the number of steps and time taken for optimization and rendering time for one image with resolution of \(648, 960\) in ETH3D~\cite{schops2017multi} training scenes. All timings are measured with the same device using single NVidia A40 GPU.
% }
% \label{tab:opt}
% \end{small}
% \end{table}

\begin{table}[t]
\centering
\begin{small}
\caption{
    \textbf{Training and Inference Time.} We report the number of steps and time taken for optimization and rendering time for one image with resolution of \(640, 960\) in ETH3D~\cite{schops2017multi} training scenes. All timings are measured with the same device using single NVidia A40 GPU. The fast training and the rendering time comes from the architectural choice~\cite{lee2022qff}. 
}
% \renewcommand{\arraystretch}{0.9}
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{@{}c|c@{\hspace{2em}}c@{\hspace{2em}}c@{}}
    \toprule
    % header
    Model & \# Steps & Training~(hh:mm) & Inference~(ss) \\
    \midrule
    FreeNeRF~\cite{yang2023freenerf} & 200,000 & 14:26 & 36.4\\
    RegNeRF~\cite{niemeyer2022regnerf} & 200,000 & 07:00 & 30.4\\
    MonoSDF~\cite{yu2022monosdf} & 200,000 & 20:54 & 136.0 \\
    Neuralangelo~\cite{li2023neuralangelo} & 200,000 & 19:58 & 61.9 \\
    Ours & 50,000 & 02:15 & 4.6 \\
    \bottomrule
\end{tabular}
}
% \vspace{-2em}
\label{tab:opt}
\end{small}
\end{table}


==> tables/tnt_advanced.tex <==
\begin{table*}[h]
\begin{small}
\centering

% \resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc}
\toprule
 & MonoSDF~(Grid) & MonoSDF~(MLP) & Ours \\
\midrule
Auditorium & 3.17 & 3.09 & \\
Ballroom & 3.70 & 2.47 & \\
Courtroom & 13.75 & 10.00 & \\
Museum & 5.68 & 5.10 & \\
\midrule
Mean & 6.58 & 5.165 & \\
\bottomrule
\end{tabular}
% }
\caption{
    \textbf{Comparison of MonoSDF~\cite{yu2022monosdf} in TNT advaced scenes}
    We evaluate the
    reconstructed point clouds using the official server and report the F-score with 10mm. Our metehod outperforms MonoSDF on all scenes. Numbers of MonoSDF are reported by the original paper.
}
\label{tab:tnt_adv}
\end{small}
\end{table*}



==> tables/tnt_training.tex <==
\begin{table}[h]
\centering
\resizebox{.48\textwidth}{!}{

\begin{tabular}{c|ccc}
\toprule
& Meetingroom & Barn & Courthouse  \\
 % &  & Barn & Church & Meetingroom & Courthouse  \\ 
% Patch. & Mono. &Novel. & Restr. &
\midrule
% none
 Ours & 21 & 46 & 35  \\
% cull
 Neuralangelo & 32 & 70 & 28  \\
\bottomrule
\end{tabular}
}
\caption{
    \textbf{Comparison on TnT~\cite{knapitsch2017tanks} dataset training scenes}.    
}
\label{tab:tnt_comp_train}
\end{table}
\vspace{-0.2in}


==> tex/introduction_backup.tex <==
% \input{figures/teaser_fig}
\section{Introduction}

Modeling 3D scenes from imagery is a core problem in computer vision, directly useful for mapping, facility assessment, robotics, construction monitoring, and more.  These applications require both accurate geometry and realistic visualization from novel views, and may involve large scenes with sparse views.

Neural Radiance Field~(NeRF)~\cite{mildenhall2021nerf} approaches can synthesize novel views with high fidelity, especially when interpolating training views. The NeRF approach also has great potential for 3D geometry estimation, as a single model can be optimized according to many losses and constraints, encoding photometric consistency, single-view predictions, and material properties. However, this potential is currently unrealized --- even  regularized approaches like RegNeRF~\cite{niemeyer2022regnerf} and FreeNeRF~\cite{yang2023freenerf} produce poor geometry and view extrapolation for challenging multiview stereo (MVS) benchmarks such as ETH3D~\cite{schops2017multi}. While traditional MVS methods currently lead such benchmarks, they have many limitations, such as modeling incomplete surfaces, low ability to render novel views, and reliance on complex algorithms and heuristics that inhibit further improvement.  Thus, it is worthwhile to explore how to make NeRF approaches more geometrically accurate.
% MVS methods currently produce better geometry in many settings, but often produce noisy and incomplete models, and it is difficult to improve MVS methods by adding more cues and priors, due to their heuristics and algorithmic complexity. 
%While MVS methods typically produce superior geometry in numerous contexts, they often result in noisy and incomplete models, and they do not support high-quality rendering. Furthermore, enhancing MVS methods by introducing additional cues and priors is challenging due to the inherent heuristics and algorithmic complexity.


%In this paper, we aim to improve the geometric accuracy of NeRF models by incorporating patch-based consistency measures,  guidance from monocular depth and surface normal predictions, and virtual source images. Our work differs from most NeRF-based work in our emphasis on obtaining accurate 3D geometry, even from larger scenes with sparse views. While some works apply NeRF modeling as a post-process to MVS, we are interested in the potential of NeRF as a self-contained solution to accurately model geometry with ability to realistically synthesize interpolated and extrapolated views.

%based approaches have shown tremendous success in novel view synthesis. 
Recent neural field based works have led to some improvements in geometric fidelity and the capability to handle sparse views~\cite{niemeyer2022regnerf, zhang2022nerfusion, jain2021putting_nerf_on_a_diet, yang2023freenerf}. 
MonoSDF~\cite{yu2022monosdf} incorporates monocular surface normal and depth predictions in a signed distance function (SDF) model. 
This works well for objects or small indoor scenes, but due to the initialization with a sphere, smoothness priors, and volumetric representation, this approach does not readily provide good results for large scenes, open scenes, or those with fine structures like bicycle racks. 
Neuralangelo~\cite{li2023neuralangelo} improves SDF modeling with coarse-to-fine optimization regularized by a surface curvature loss, which can accurately model details in densely viewed scenes, but our experiments indicate limited effectiveness in a sparse view setup. 
RegNerf~\cite{niemeyer2022regnerf} incorporates losses of appearance likelihood and smooth depth for patches on randomly sampled virtual views, improving results when sparse input views are available.  
%.  Yet, our experiments show as our experiments show, this virtual view patch-based regularization is not sufficient to achieve geometrically accurate models.  
While not complete solutions, these approaches contain two critical ideas that we will build on: (1) leverage monocular surface normal and depth predictions to guide the model; (2) encourage virtual view appearance consistency to further regularize the model.   
%  Monocular predictions of surface normal and up-to-scale depth are not easily incorporated into the ray-based optimization for density models. 


%Yet, NeRF based approaches fails to generate good extrapolating views~\cite{} on wide-baseline settings, partly due to that it does not reconstruct reliable 3D geometry compared to traditional 3D reconstruction approaches such as Multi-View Stereo~(MVS)~\cite{}. 
%Recently, few methods has addressed the problems in these wide-baseline scenes by adding randomized novel view sampling~\cite{regnerf}, altering frequencies~\cite{freenerf} and using sparse-to-dense depth supervision ~\cite{ddsnerf}.
%These methods show success in object centric or front-facing sparse view setting such as DTU~\cite{dtu} or LLFF~\cite{llff}, but does not scale well to real-world datasets such as ETH3D High-resolution benchmark.

In this paper, we aim to create 3D models that provide accurate geometry and view synthesis, using a patch-based approach that effectively leverages monocular depth/normal predictions and virtual view appearance consistency priors.  
% We find that density-based models are better suited to encoding details in large scenes, compared to SDF-based models, but it is difficult to incorporate monocular predictions of surface normal and up-to-scale depth in ray-based sampling of density models, since the surface normal and relative depth are not well-defined along a single ray.  With patch-based sampling, we make more effective use of these monocular cues.  \shenlong{half sentence on why}
% Further, patch-based sampling enables losses based on normalized cross-correlation (NCC) and structural similarity (SSIM), which are widely used in classic MVS due to their robustness to contrast changes and lighting effects.  These measures increase efficacy of constraints based on patches from randomly sampled novel views.  \shenlong{this sentence is confusing; and it's not clear you have used it for photometric consistency}
We have found that density-based models are better suited for encoding details in large scenes compared to SDF-based models. However, integrating monocular predictions of surface normal and up-to-scale depth into the ray-based sampling of density models is difficult because surface normal and relative depth are not well-defined along a ray in the density model. With our patch-based sampling technique, we use these monocular cues more effectively. % \shenlong{add half sentence saying why}
Additionally, patch-based sampling allows us to take advantage of structural losses for regularization, such as normalized cross-correlation (NCC) and structural similarity (SSIM). These are robust to varying lighting conditions, hence extensively employed in classic MVS. Using these losses, we encourage patch-level photometric consistency across randomly sampled virtual views. % \shenlong{revised for clarity, please check if they make sense}
Density-based models may ``cheat'' by modeling view-dependent effects as densities near the frustrum. We prevent this and further regularize geometry by restricting non-zero densities to be loosely consistent with the monocular depth predictions, after they are translated/scaled based on structure-from-motion (SfM) points. This ``density restriction'' greatly improves geometric accuracy, with a slight drop in novel view synthesis metrics.    
With these improvements, our method outperforms on other NeRF-based methods on the ETH3D benchmark~\cite{schops2017multi} in both novel view synthesis and geometry estimation. We also achieve competitive results on the Tanks and Temples benchmark~\cite{knapitsch2017tanks}. Though falling short of state-of-art classic MVS methods, such as ACMMP~\cite{Xu2022Multi}, in point cloud metrics, our results support the potential of NeRF-based approaches to eventually surpass traditional MVS approaches.

In summary, this paper offers the following \textbf{contributions}:
\begin{itemize}
\item We demonstrate the effective use of monocular surface normal and relative depth predictions for density-based NeRF models, patch-based ray sampling and occupancy constraints. 
\item Enabled by patch-based sampling, we demonstrate the effectiveness of photometric consistency (NCC, SSIM) between virtual and training views and local geometric consistency with monocular estimates.
% \item Our method significantly improves in geometric accuracy, e.g. {\bf 4x over RegNeRF} and {\bf 2x over MonoSDF} on average F1@2cm for ETH3D MVS benchmark and achieves competitive novel view synthesis ({\bf best in SSIM and LPIPS}). This result indicates a fruitful research direction to improve the geometric accuracy of NeRF-based models, e.g., by incorporating additional monocular predictions, material models, and other variables and priors.
\item Our method significantly improves geometric accuracy, achieving {\bf 4x the performance of RegNeRF} and {\bf 8x that of FreeNeRF} on average F1@2cm for the ETH3D MVS benchmark and produces competitive results in novel view synthesis, ranking {\bf best in terms of SSIM and LPIPS}. These findings indicate a fruitful research direction to improve the geometric accuracy of NeRF-based models.
\end{itemize}

%In this paper, we explore ways to regularize NeRF geometry by proposing photometric and geometric constraints in the NeRF optimization process using patches and monocular geometric priors. We show that our method allows photo-realistic reconstruction of sparse view, wide-baseline scenes. 
%We first show that patch based training of monocular geometric prior translates geometric details in regions with high-gradients.
%Next, we propose enforcing photometric consistency between randomly sampling views and training views show an effective strategy to regularize appearance and geometry. 
%Finally, we show that pruning out empty spaces using monocular and sparse geometry reduces variance in reconstructed geometry. 
%With these improvements, we achieve promising results on ETH3D benchmark, outperforming the baselines by huge margin in both appearance and geometry, and show a promising direction of replacing the MVS with the NeRF optimization. 
%We show real-time rendering of these photo-realistic scenes on a web-browser using QFF~\cite{qff} for interactive demonstration. 

%In summary, our main contributions are as following:
%\begin{itemize}
%    \item Patch-based formulation of monocular geometric prior distillation
%    \item Simple and effective novel view patch sampling and photometric loss
%    \item Empty space pruning to resolve floaters and background collapse
%\end{itemize}

==> tex/method_backup.tex <==

\section{Method}
% We start by reviewing the NeRF and introducing the notations used throughout the paper.  Then, we cover each component of our main contributions. Our method contains three main components: 1) using monocular geometric priors with patch-based formulation, 2) Randomly sampled views for photometric consistency-driven regularization, and 3) empty space pruning with monocular depth and sparse geometry.  We provide a visualization of the overview of our architecture in Figure~\ref{fig:architecture}. 

Given a collection of posed images capturing a large scale scene, our goal is to construct a 3D neural radiance field that renders high-quality images and predicts accurate and complete surface geometry. We achieve this by introducing three novel components: 1) \textbf{patch-based geometry supervision} to better leverage the local consistency of monocular cues; 2) \textbf{patch-based occlusion-aware photometric regularization} across virtual and training viewpoints, better guiding NeRF training when input views are sparse; 3) \textbf{density restriction} through monocular geometry estimates and sparse points, inhibiting NeRF from modeling view-dependent effects with densities in unlikely areas. Figure~\ref{fig:architecture} provides a summary of our approach.



\subsection{NeRF with Patch-Based Sampling}
\label{sec:nerf}

The Neural Radiance Field (NeRF)~\cite{mildenhall2020nerf} establishes a parametric representation of the scene, enabling realistic rendering of novel viewpoints from a given image collection. NeRF is defined by $\mathbf{c}, \sigma = F_\theta(\mathbf{x}, \mathbf{v})$, where $\mathbf{c}$ is output color, $\sigma$ represents opacity, $\mathbf{x}$ is the 3D point position, and $\mathbf{v}$ denotes the viewing direction. The variable $\theta$ represents learnable parameters optimized for each scene. 
The pixel color and depth can be computed through volume rendering along the corresponding ray $\mathbf{r}(t) = \mathbf{o} + t\mathbf{v}$, where $\mathbf{o}$ is the camera center and $\mathbf{v}$ is the ray direction.


% Considering an input query viewpoint with camera parameters $\mathbf{K}$, $\mathbf{R}$, and $\mathbf{t}$ (representing intrinsic parameters, rotation, and translation), a pixel's camera viewing ray can be calculated as $\mathbf{r}(t) = \mathbf{o} + t\mathbf{v}$, where $\mathbf{o}$ is the camera center and $\mathbf{v}$ is the ray direction. 
% The pixel color is then computed through volume rendering as $\mathbf{c}(\mathbf{r}) = \sum_{i=1}^{N}w_i\mathbf{c}_i$, with $\mathbf{c}_i$ being the NeRF color evaluated from the i-th sampled point $\mathbf{x}_i = \mathbf{o} + t_i\mathbf{v}$ along the ray. Weight $w_i$ is calculated through alpha composition as $w_i = \text{exp} \left(-\sum_{j=1}^{i-1}\sigma_j\delta_j \right)(1-\text{exp}(-\sigma_i\delta_i))$, where $\sigma_i$ defines sampled point's opacity and $\delta_i = t_{i} - t_{i-1}$ defines the distance between the $i$-th sample and its preceding point. The depth of each pixel can also be rendered through volume rendering: $\mathbf{d}(\mathbf{r}) = \sum^n_{i=1} \hat{w}_i t_i$, where $\hat{w}_i$ is the weight normalized along the ray. 

NeRF is trained by minimizing the difference between the rendered RGB value $\hat{\mathbf{c}}$ and the observed value $\mathbf{c}$ of random sampled pixels across images.
Despite its exceptional performance in synthesizing nearby novel views, NeRF falls short in capturing high-quality geometry and rendering extrapolated viewpoints~(Figure~\ref{fig:eth_mesh_comp}). 
To overcome these challenges, we sample local patches instead of discrete rays during training, and propose our patch-based supervision and regularization, in addition to per-pixel Huber Loss~$L_\text{huber}(\hat{\mathbf{c}}, \mathbf{c})$ for RGB supervision.

 


% \subsection{Distillation of monocular geometric priors with patches}
\subsection{Distillation of Patch-based Monocular Cues}
\label{sec:monocular}

Learning-based networks for single-image normal and depth prediction can provide robust cues for the geometry, especially for areas with photometric ambiguity~(reflective and textureless surfaces). 
Taking inspiration from this, prior works~\cite{guo2022neural,yu2022monosdf} exploit monocular depth and normal supervision for neural fields, and apply a pixel-based scale and shift per batch to align monocular and predicted depth.
% However, monocular methods tend to be consistent locally, and the global transformed depth will not provide optimal supervision for pixels randomly sampled from the whole image.
However, monocular methods tend to be only locally consistent.
% Scale-and-shift solved with pixels sampled from the whole image would be less accurate than that solved locally, and thus the transformed depth would not provide optimal supervision.
Image-wide scale-and-shift alignment may still leave large depth errors that reduce the usefulness of monocular depth estimates for supervision.
To address this challenge, we compute the scale and shift per local patch to better leverage the capacity of monocular cues and achieve better performance~(Compare \textit{Mono.} and \textit{Mono.+Patch} in Tables~\ref{tab:ablation} and~\ref{tab:tnt}).

Given a patch $P=\{p\}$, we compute the transformed monocular depth $\{ d_p^\dag \}$ using the optimal scale $s$ and shift $t$ from a least-squares criterion~\cite{manivasagam2020lidarsim} between rendered depth$\{ \hat{d}_p \}$ and monocular depth $\{ d_p \}$ on $P$.
The depth loss $L_\text{depth}$ and $L_{\nabla \text{depth}}$ are applied to penalizes the absolute and gradient discrepancy between $\{ \hat{d}_p \}$ and $\{ {d}_p^\dag \}$:

\begin{align}
L_\text{depth} &= \sum_{p \subset P} \| \hat{d}_p - {d}_p^{\dag} \| \\
L_{\nabla \text{depth}} &= \sum_{p \subset P} \| \nabla \hat{d}_p - \nabla {d}_p^{\dag} \| ,
\end{align}

% \[
% \resizebox{\columnwidth}{!}{
% L_\text{depth} = \sum_{Q \subset P} \sum_{p \in Q} \| \hat{d}_p - {d}_p^Q \|, L_{\nabla \text{depth}} = \sum_{Q \subset P} \sum_{p \in Q} \| \nabla \hat{d}_p - \nabla {d}_p^Q \|,
% }
% \]

% where $d_p^\dag = s d_p + t$ represents the normalized depth using the optimal scale $s$ and shift $t$ estimated from pixels $\{p\}$ with a least-squares criterion~\cite{manivasagam2020lidarsim}, and $\nabla {d}_p$ is the gradient value of depth image at pixel $p$. 
% \[
% {d}_p^Q = s_Q {d}_p + t_Q
% \text{, \ \ where \ \ }
% t_Q = \frac{1}{|Q|}\sum_{p \in Q} {d}_p - \hat{d}_p, 
% s_Q = \frac{\sum_{p \in Q} {d}_p}{\sum_{p \in Q} {d}_p - t_Q}
% \]

% \begin{gather}
% {d}_p^Q = s_Q {d}_p + t_Q, \nonumber \\
% \text{where} (s, t) = \argmin_{s,t} \sum_{i=1}^{M} (s d_i + t - d_i^\ast)^2 
% \end{gather}

% \begin{align}
% {d}_p^Q = s_Q {d}_p + t_Q, \nonumber \\
% \text{where} \ \ t_Q = \frac{1}{|Q|}\sum_{p \in Q} {d}_p - \hat{d}_p, 
% s_Q = \frac{\sum_{p \in Q} {d}_p}{\sum_{p \in Q} {d}_p - t_Q}
% \end{align}

Following RefNeRF~\cite{verbin2022ref}, we compute density-based normals $\mathbf{n}^\nabla_i = -\nabla \sigma_i / \|-\nabla \sigma_i\|$ with the gradient of opacity and MLP-based normals ${\mathbf{n_i}}^\theta=F_\theta(\mathbf{x_i}, \mathbf{v_i})$ with a normals rendering head. 
After volume rendering, the two normals predictions are supervised with monocular normals $\{{n}_p\}$ using angular and $L_1$ loss:
% We also apply a normal loss with the monocular estimation normals $\mathbf{n}$ to regularize our rendered density field, following RefNeRF~\cite{verbin2022ref}. 
% Like their approach,  we define two separate formulations of rendered surface normals. 
% First, we apply an additional normal rendering MLP head on NeRF. Using this MLP head our NeRF can produce per-ray normal estimation with volume rendering: 
% per-sample surface normal using MLP, 
% denoted as $\mathbf{n}^\theta_i$, which are rendered based on rendering equation as 
% ${\mathbf{n}}^\theta = \sum_i w_i \mathbf{n}^\theta_i$. 
% Next, we estimate surface normal as the negative direction of the gradient of the optical density, denoted as $\mathbf{n}^\nabla_i = -\nabla \sigma_i / \|-\nabla \sigma_i\|$, with rendered form as ${\mathbf{n}}^\nabla = \sum_i w_i \mathbf{n}^\nabla_i$.
% We directly supervise ${\mathbf{n}}^\theta, {\mathbf{n}}^\nabla$ with the monocular surface normal estimate $\hat{\mathbf{n}}$ as:



\begin{equation}
\begin{split}
L_\text{normal} &= \sum_{p \subset P} (1 - \cos({\mathbf{n}}_p, \mathbf{n}^\nabla_p) + |{\mathbf{n}}_p - \mathbf{n}^\nabla_p|) \\
&+ \sum_{p \subset P} (1 - \cos({\mathbf{n}}_p, \mathbf{n}^\theta_p) + |{\mathbf{n}}_p - \mathbf{n}^\theta_p|)
\end{split}
\end{equation}

We also apply the gradient loss $L_{\nabla \text{normal}}$ over $\mathbf{n}^\nabla$: 
\begin{equation}
\begin{split}
L_{\nabla \text{normal}} &= \sum_{p \subset P} (|\nabla {\mathbf{n}}_p - \nabla \mathbf{n}^\nabla_p|)
\end{split}
\end{equation}

Finally, our patch-based monocular loss is defined as: 
\begin{equation}
    L_\text{mono} = L_\text{depth} + L_{\nabla \text{depth}} + L_\text{normal} + L_{\nabla \text{normal}}.
\end{equation}

\subsection{Patch-based Photometric Consistency over Virtual Views}
\label{sec:regularization}

% \subsection{Photometric Consistency Regularization through Novel View Patch Sampling}

NeRF models are under-constrained when the input images are sparse, and create artifacts in novel view renderings despite a low training view loss~(overfitting). 
To add additional regularization, we enforce an occlusion-aware photometric consistency between training patches and randomly sampled virtual patches.
% To add additional constraints, RegNeRF~\cite{niemeyer2022regnerf} samples virtual patches, and enforces planar assumption with depth smoothing loss and RGB likelihood loss with a pretrained color adversarial model.
% However, both regularization are not leveraging the context of the scene, but enforcing general prior and assumption.
% We interpret the regularization problem as how to use training views information to guide test views rendering. 
% If we know the test view poses, we can enforce the photometric consistency between the training patches and test patches with patch wrapping like MVS. 
% Though the test view poses are unknown during the training time, we can randomly sample virtual patches close to the existing training views to serve as a strong regularization for the appearance and geometry consistency. 
Though designed for sparse-view input, we find that the photometric regularization works for general setups, significantly boosting the performance for both sparse-view~(Table~\ref{tab:ablation}) and dense-view scenes~(Table~\ref{tab:tnt}).

\input{figures/novel_patch}

As visualized in Fig.~\ref{fig:nvp}, for each training patch $P$, we randomly sample a corresponding virtual camera center $o_{p^\ast}$ within a fixed distance to $o_p$~($0.05 \times$ the scene width). 
The correspondence is determined by unprojecting the pixel from the training view into 3D points, denoted as $\mathbf{X}_p = \mathbf{o}_p + \hat{d}_p\mathbf{v}_p$, and then back-projecting $\mathbf{X}_p$ into the $\mathbf{o}_{p^\ast}$ for the corresponding direction $\mathbf{v}_{p^\ast} = (\mathbf{X}_p - \mathbf{o}_{p^\ast}) / \|(\mathbf{X}_p - \mathbf{o}_{p^\ast})\|$. 
Given $\mathbf{o}_{p^\ast}$ and $\mathbf{v}_{p^\ast}$, we render the color $\mathbf{\hat{c}}_{p^\ast}$ and depth ${\hat{d}}_{p^\ast}$ for virtual patch $P^\ast$.
Since viewing the same point from different perspectives can result in varying occlusion patterns, we additionally apply mask $M_{p\rightarrow p^\ast}$ to remove any clearly occluded pixels to eliminate the occlusion impact.  
We compute $M_{p\rightarrow p^\ast}$ by comparing an angle threshold $\theta_{\text{thresh}}$ and the angle $\theta_{p^\ast \rightarrow p}$ between rays from $\mathbf{o}_p$ to $\mathbf{X}_p$ and $\mathbf{o}_p$ to $\mathbf{X}_{p^\ast}$:
\begin{equation}
\begin{split}
\theta_{p^\ast \rightarrow p} &= \arccos(\mathbf{v}_{p^\ast \rightarrow p} \cdot \mathbf{v}_p), \\
M_{p\rightarrow p^\ast} &= 
  \begin{cases} 
   1 & \text{if } \theta_{p^\ast \rightarrow p} \leq \theta_{\text{thresh}} \\
   0 & \text{otherwise}
  \end{cases} \\
\end{split}
\end{equation}
where $\mathbf{v}_{p^\ast \rightarrow p} = \frac{(\mathbf{X}_{p^\ast}  - \mathbf{o}_{p})}{\|(\mathbf{X}_{p^\ast}  - \mathbf{o}_{p})\|}$ and $
\mathbf{X}_{p^\ast} = \mathbf{o}_{p^\ast} + \hat{d}_{p^\ast}\mathbf{v}_{p^\ast}$.

The occlusion-aware patch-based consistency loss is defined as:
\begin{equation}
\begin{split}
L_\text{virtual} &= L_\text{SSIM}(\{\mathbf{\hat{c}}_{p^\ast}\}, \{{\mathbf{c}}_p\}, \{M_{p\rightarrow p^\ast}\}) \\
&+ L_\text{NCC}(\{\mathbf{\hat{c}}_{p^\ast}\}, \{{\mathbf{c}}_p\}, \{M_{p\rightarrow p^\ast}\})
\end{split}
\end{equation}

where $L_\text{SSIM}$ and $L_\text{NCC}$ measure the structural similarity and normalized cross-correlation between two masked patches respectively.
Both losses are robust to view-dependent effects like illumination change.
Though we rely on rendered depth for the loss, the occlusion mask will inhibit the loss from incorrectly guide the optimization in the beginning.



\subsection{Density Restriction by Empty Space Pruning with Sparse SfM Geometry}
\label{sec:pruning}
One significant challenge in NeRF is the occurrence of floaters and background collapse~\cite{barron2022mip}.
The challenge arises because NeRF fails to predict correct geometry for surfaces with low texture and view-dependent effects, or tends to overfit in near-camera regions that are unseen from other views during training.  
We address this problem by limiting the domain of density distributions using monocular geometric prior and sparse multi-view prior~(Figure~\ref{fig:empty_space_pruning}).

Monocular depth provides useful relative distance information, and SfM points provide metric depth that can be utilized for aligning the monocular depth with 3D space. 
For each view, we use RANSAC to solve a scale and shift for monocular depth with the projected sparse points to minimize the influence of noise in the points. 
We then constrain the grid density distribution to a specified interval around the estimated depth along each ray. 
This hard restriction effectively prunes out empty space, thereby eliminating the floaters and improving the overall geometry estimation.

\input{figures/empty_space_pruning}

\subsection{Training}
\label{sec:training}
We start by estimating monocular geometric cues with images using the pretrained Omnidata~\cite{eftekhar_iccv2021_omnidata} model. 
With the sparse points from SfM, we use RANSAC to find the optimal shift and scale for the monocular depth for density restriction. 
To initialize the density restriction, we voxelize the space, project the center of each voxel to all training views, label voxels with centers lying within 20\% of any monocular depth map, and exclude sampling outside of labeled voxels.
During training, we iterate through images, sample a batch~(128) of $8\times8$ patches per reference image, sample one virtual patch for each training patch, and evaluate the loss terms for all patches.
We use NerfAcc~\cite{li2022nerfacc} with modified QFF~\cite{lee2022qff} as our base model for faster training and inference without loss of accuracy, and train with the unified loss $L = \sum \lambda_{:} L_{:}$, with $\lambda_{\text{huber}} = 1.0$, $\lambda_{\text{depth}} = 0.05$, $\lambda_{\nabla \text{depth}} = 0.025$, $\lambda_{\text{normal}} = 1 \times 10^{-3}$, $\lambda_{\nabla \text{normal}} = 5 \times 10^{-4}$, $\lambda_{\text{SSIM}} = 1 \times 10^{-4}$, $\lambda_{\text{NCC}} = 1 \times 10^{-4}$. 
Please see our supplementary material for more details on parameters and model architecture.




